PerceptionCLIP: Visual Classification by Inferring and Conditioning on Contexts

Vision-language models like CLIP are widely used in zero-shot image classification due to their ability to understand various visual concepts and natural language descriptions. However, how to fully leverage CLIP's unprecedented human-like understanding capabilities to achieve better performance is still an open question. This paper draws inspiration from the human visual perception process: when classifying an object, humans first infer contextual attributes (e.g., background and orientation) which help separate the foreground object from the background, and then classify the object based on this information. Inspired by it, we observe that providing CLIP with contextual attributes improves zero-shot image classification and mitigates reliance on spurious features. We also observe that CLIP itself can reasonably infer the attributes from an image. With these observations, we propose a training-free, two-step zero-shot classification method PerceptionCLIP. Given an image, it first infers contextual attributes (e.g., background) and then performs object classification conditioning on them. Our experiments show that PerceptionCLIP achieves better generalization, group robustness, and interoperability. Our code is available at https://github.com/umd-huang-lab/perceptionCLIP

==> sections/08_ack.tex <==
\section*{Acknowledgments}
\label{sec:ack}

An, Zhu, and Huang are supported by National Science Foundation NSF-IIS-FAI program, DOD-ONR-Office of Naval Research, DOD Air Force Office of Scientific Research, DOD-DARPA-Defense Advanced Research Projects Agency Guaranteeing AI Robustness against Deception (GARD), Adobe, Capital One and JP Morgan faculty fellowships.

==> tables/factor_2.tex <==

\begin{table*}[!ht]
\centering
\small
\caption{Zero-shot classification accuracy on five datasets. We use ViT-B/16 CLIP model and the one-step inference method. The first part shows the results used in \cite{radford2021learning}. The second part shows the result of considering one contextual attribute. The highest performance is in bold for each dataset, and the next two highest values are underlined. The third part shows the result of using compositions of contextual attributes. The best performance is highlighted in bold. Results show that considering only one attribute at inference time can achieve comparable performance as using 80 templates and composing factors further improves performance.}
\resizebox{0.95\textwidth}{!}{\begin{tabular}{llccccc}
\toprule
\multicolumn{2}{c}{\textbf{Attributes}}                            & \textbf{ImageNet}             & \textbf{ImageNetV2}           & \textbf{ImageNet-R}            & \textbf{ImageNet-A}            & \textbf{ImageNet-Sketch}       \\ \midrule
\multicolumn{2}{c}{single template}                    & 66.72\%              & 60.85\%              & 73.99\%              & 47.80\%              & 46.16\%              \\
\multicolumn{2}{c}{80 templates}                       & 68.32\%              & 61.93\%              & 77.71\%              & 49.95\%              & 48.26\%              \\ \midrule
\multirow{11}{*}{single factor} & background   & 67.48\% & \textbf{61.60\%} & 75.75\% & 48.99\% & 47.12\% \\
                                & illumination & 66.94\% & 60.90\% & 75.01\% & 48.16\% & 46.23\% \\
                                & orientation  & 67.32\% & 60.99\% & 74.50\% & 48.28\% & 46.84\% \\
                                & quality      & \ul{67.99\%} & \ul{61.45\%} & \ul{76.34\%} & \textbf{50.11\%} & \ul{47.50\%} \\
                                & quantity     & \ul{67.71\%} & \ul{61.50\%} & 75.38\% & \ul{50.01\%} & 46.73\% \\
                                & perspective  & 67.60\% & 61.20\% & 74.92\% & 49.21\% & 46.91\% \\
                                & art          & 67.33\% & 61.04\% & \textbf{77.15\%} & \ul{49.48\%} & \textbf{48.05\%} \\
                                & medium       & 67.19\% & 60.59\% & 76.38\% & 49.17\% & 46.75\% \\
                                & condition    & \textbf{68.20\%} & 61.37\% & \ul{75.50\%} & 49.16\% & 47.22\% \\
                                & color-scheme & 66.50\% & 60.49\% & 73.78\% & 47.83\% & 46.61\% \\
                                & tool         & 66.68\% & 60.58\% & 75.40\% & 48.37\% & \ul{47.38\%} \\ \midrule
\multicolumn{2}{c}{composition of  top 2 factors}          & \textbf{68.35\%}              & 61.67\%              & 77.88\%              & \textbf{50.83\%}    & 48.11\%              \\
\multicolumn{2}{c}{composition of  top 3 factors}          & 68.26\%     & 61.89\%     & 77.65\%     &50.42\%               & 48.41\%     \\ 
\multicolumn{2}{c}{composition of  top 4 factors}          & 68.22\%  & \textbf{61.98\%}  &  \textbf{78.04\%}  & 50.49\% & \textbf{48.72\%}\\
\bottomrule
\end{tabular}}\label{tab:main_results_2}
\end{table*}


==> tables/factors.tex <==

\begin{table*}[t]
\centering
\small
\caption{
Zero-shot classification accuracy on five datasets using ViT-B/16. The best result in each column is highlighted in bold, while the next two highest values are underlined.
}
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{llccccc}
\toprule
\multicolumn{2}{c}{\textbf{Attributes}}                            & \textbf{ImageNet}             & \textbf{ImageNetV2}           & \textbf{ImageNet-R}            & \textbf{ImageNet-A}            & \textbf{ImageNet-Sketch}       \\ \midrule
\multicolumn{2}{c}{single template}                    & 66.72\%              & 60.85\%              & 73.99\%              & 47.80\%              & 46.16\%              \\
\multicolumn{2}{c}{80 templates}                       & 68.32\%              & 61.93\%              & 77.71\%              & 49.95\%              & 48.26\%              \\ \midrule
\multirow{11}{*}{single attribute} & background           & 67.70\%              & \textbf{61.91\%}        & 75.71\%              & 49.13\%              & 47.21\%              \\
                                & illumination         & 66.91\%              & 61.04\%              & 74.60\%              & 48.32\%              & 46.08\%              \\
                                & orientation          & 67.21\%              & 61.04\%              & 74.31\%              & 47.88\%              & 46.54\%              \\
                                & quality              & \ul{68.11\%}        & \ul{61.78\%}        & \ul{76.24\%}        & \textbf{50.41\%}        & \ul{47.39\%}        \\
                                & quantity             & 67.57\%              & 61.39\%              & 75.22\%              & \ul{50.08\%}        & 46.57\%              \\
                                & perspective          & \ul{67.87\%}        & 61.36\%              & 74.91\%              & 49.55\%              & 46.90\%              \\
                                & art                  & 67.42\%              & 60.94\%              & \textbf{77.08\%}        & \ul{49.59\%}        & \textbf{47.95\%}        \\
                                & medium               & 67.22\%              & 60.73\%              & \ul{76.30\%}        & 49.45\%              & 46.78\%              \\
                                & condition            & \textbf{68.30\%}        & \ul{61.64\%}        & 75.51\%              & 49.25\%              & \ul{47.25\%}        \\
                                & color-scheme         & 66.67\%              & 60.70\%              & 73.85\%              & 48.07\%              & 46.41\%              \\
                                & tool                 & 66.70\%               & 60.61\%               & 75.32\%             & 48.28\%             & 47.22\%             \\ \midrule
\multicolumn{2}{c}{composition of  top 2 attributes}          & 68.49\%              & 61.95\%              & 77.64\%              & 50.85\%     & 48.18\%              \\
\multicolumn{2}{c}{composition of  top 3 attributes}          & \textbf{68.52\%}     & 62.01\%     & 77.92\%     & 50.53\%               & 48.39\%     \\ 
\multicolumn{2}{c}{composition of  top 4 attributes}          & 68.50\%     & \textbf{62.24\%}     & \textbf{77.95\%}     & \textbf{50.97\%}               & \textbf{48.79\%}     \\ 
\bottomrule
\end{tabular}}\label{tab:main_results}
\end{table*}

==> tables/intervention.tex <==
\begin{table}[h]
\centering
\small
\caption{Comparing two-step inference (inference w/ intervention) with one-step inference (inference w/o intervention). All the results are tested with ViT-B/16 CLIP model using 80 templates.}
\begin{tabular}{llllll}
\toprule
 \multirow{2}{*}{} & \textbf{Without} & \multicolumn{2}{c}{\textbf{With intervention}}                                            \\\cline{3-4}
                  &      \textbf{intervention}               & \textbf{ClassAtrr} & \textbf{PureAttr} \\
\midrule
ImageNet & 68.32\% & 68.50\% & \textbf{68.56\%} \\
ImageNetV2 & 61.93\% & \textbf{62.24\%} & \textbf{62.24\%} \\
ImageNet-R & 77.71\% & \textbf{77.83\%} & 77.53\% \\
ImageNet-A & 49.95\% & \textbf{50.37\%} & 50.35\% \\
ImageNet-Sketch & \textbf{48.26\%} & 48.18\% & 48.22\% \\
\bottomrule
\end{tabular} \label{tab:compare_1}
\end{table}
